Sparse and Private Distributed Matrix Multiplication with Straggler Tolerance

This paper considers the problem of outsourcing the multiplication of two private and sparse matrices to untrusted workers. Secret sharing schemes can be used to tolerate stragglers and guarantee information-theoretic privacy of the matrices. However, traditional secret sharing schemes destroy all sparsity in the offloaded computational tasks. Since exploiting the sparse nature of matrices was shown to speed up the multiplication process, preserving the sparsity of the input matrices in the computational tasks sent to the workers is desirable. It was recently shown that sparsity can be guaranteed at the expense of a weaker privacy guarantee. Sparse secret sharing schemes with only two output shares were constructed. In this work, we construct sparse secret sharing schemes that generalize Shamir's secret sharing schemes for a fixed threshold $t=2$ and an arbitrarily large number of shares. We design our schemes to provide the strongest privacy guarantee given a desired sparsity of the shares under some mild assumptions. We show that increasing the number of shares, i.e., increasing straggler tolerance, incurs a degradation of the privacy guarantee. However, this degradation is negligible when the number of shares is comparably small to the cardinality of the input alphabet.

==> leakage_optimality.tex <==
The authors of \cite{xhemrishi2022efficient} showed numerically that for a sparse secret sharing scheme with two shares with sparsities $\sr$ and $\sar$, the minimal leakage is obtained for $\bfR$ and $\bfA+\bfR$ having the same desired sparsities $\sr=\sar$. This result will be proven analytically in the following.

In its essence, sparsity in the secret shares is preserved by dependently designing the random matrix $\rvR$ on the input matrix $\rvA$. While the dependency ensures sparsity, it will introduce an information leakage. This could be avoided by generating $\rvR$ uniformly at random from $\Fq$, thus leading to dense shares $\rvR$ and $\rvA+\rvR$.

For desired sparsity levels of $\rvR$ and $\rvA+\rvR$, the authors of \cite{xhemrishi2022efficient} proposed a suitable probability distribution of $\rvR$ that minimizes the leakage. Thereby, the authors make the assumption of the entries $\rvA_{\{i,j\}}$ of $\rvA$ being independent among each other, hence also the entries of $\rvR$. Designing the probability distribution comes down to finding $p_{r,a} \triangleq \Pr(\rvR_{\{i,j\}} = r|\rvA_{\{i,j\}} = a)$ for all $r,a \in \mathbb{F}_q$ under constraints. First, the $p_{r,a}$'s have to form a probability distribution, and second, that the desired sparsities are attained by $\Pr(\rvR_{\{i,j\}} = 0) = \sum_{a\in\Fq} \pra[0][a] \cdot \pa(a) = \sr$ and $\Pr(\rvR_{\{i,j\}} + \rvA_{\{i,j\}} = 0) = \sum_{a\in\Fq} \pra[-a][a] \cdot \pa(a) = \sar$. Note that the choice of the $\pra$'s affects the leakage. To minimize the leakage, we analyze the total leakage resulting from the sum $\leakage{1}+\leakage{2}$ and show that this is equivalent to optimizing the maximum leakage.

Let $\savg$ be the desired average sparsity, i.e., $\savg\define\frac{\sr+\sar}{2}$, where the sparsities of $\sar$ and $\sr$ are given by \cref{lemma:sparsity_delta}.
\begin{lemma}\label{lemma:sparsity_delta}
We follow the rules in \cref{eq:dependent_on_0,eq:dependent_on_nz} to construct two matrices $\bfR$ and $\bfA+\bfR$ dependently on $\bfA$ with sparsity $s$. We assume that the difference in sparsities between $\sar$ and $\sr$ is $2\sdiff$. This is without loss of generality, since by construction the scheme is fully symmetric in $\sr$ and $\sar$. The sparsity levels result in
\begin{align*}
    \sr &\define \savg - \sdiff = \pz s + \pext (1-s), \\
    \sar &\define \savg + \sdiff = \pz s + \pnz(1-s).
\end{align*}
\end{lemma}

While \cite{xhemrishi2022efficient} optimize the leakage for a given $\sr$ and $\sar$, we seek to optimize the leakage for a certain average sparsity $\savg\define\frac{\sr+\sar}{2}$. Hence, we also optimize over the parameter $\sdiff$ introduced in \cref{lemma:sparsity_delta}. \cref{prop:general_optimization} states the general optimization problem required to solve to obtain the least possible leakage.
\begin{proposition} \label{prop:general_optimization}
Let $\mathcal{P} \triangleq \{p_{r,a}: r,a\in \mathbb{F}_q\}$, then the minimum leakage for a given average sparsity $\savg$ is obtained by solving the following optimization problem:
\begin{align*}
    \lossopt &= \optimizerdelta \leakage{1} + \leakage{2} = \optimizerdelta \mutinf\left(\rvR; \rvA\right) + \mutinf\left(\rvA+\rvR; \rvA\right) \\
    &=\optimizerdelta \begin{aligned}[t] &\kl{\paandr}{\pa \pr} + \kl{\paandapr}{\pa \papr} \end{aligned} \\
    &=\optimizerdelta \sum_{a,b\in\mathbf{F}_q} \pa(a) \!\left( \pra[b-a][a] \log\frac{\pra[b-a][a]}{\papr(b)} + \pra[b][a] \log\frac{\pra[b][a]}{\pr(b)} \right)\!
\end{align*}
subject to
\begin{align*}
    \forall a\in\Fq: \pra[0][a] + \sum_{r\in\Fqstar} \pra[r][a] - 1 &= 0, \\[-5pt]
    \pra[0][0] \cdot \pa(0) + \sum_{a\in\Fqstar} \pra[0][a] \cdot \pa(a) - \savg + \sdiff &= 0, \\[-5pt]
    \pra[0][0] \cdot \pa(0) + \sum_{a\in\Fqstar} \pra[-a][a] \cdot \pa(a) -\savg - \sdiff &= 0.
\end{align*}
\end{proposition}

Based on the assumption of entries in $\rvA$ being identically distribution among the non-zero entries, we investigate the same scheme as proposed in \cite{xhemrishi2022efficient}, which we give in the following:

\begin{align}
 \label{eq:dependent_on_0}
    \Pr\{\Rij = r \lvert \Aij = 0\} \!&\!= \begin{cases} 
    \pz, &r = 0 \\   \pzinv , &r \neq 0,
    \end{cases}\\
\label{eq:dependent_on_nz}
    \Pr\{\Rij = r \lvert \Aij = a\} \!&\!= \begin{cases} 
    \pext, &r = 0 \\ \pnz, &r = -a, \\
    p_{2,3}^{\text{inv}} , &r \not\in \{0,-a\}, \\
    \end{cases}
\end{align}
where $r\in \F_q$, $a \in \F_q^*$, and $-a$ is the additive inverse of $a$ in $\F_q^*$. Further, $\pz,\pext,\pnz, \pzinv \triangleq (1-\pz)/(q-1)$ and $p_{2,3}^{\text{inv}} \triangleq (1-\pext-\pnz)/(q-2)$ are non-negative numbers smaller than $1$.Numerical results have shown \cite{xhemrishi2022efficient} that given the entries of $\rvA$ being i.i.d. and the non-zero entries uniformly distributed over $\Fq^*$, optimizing over PMFs as in \cref{eq:dependent_on_0,eq:dependent_on_nz} is equivalent to optimizing over $q^2$ unknowns $\pra$. This justifies the usage of PMFs as in \cref{eq:dependent_on_0,eq:dependent_on_nz}.Under this model, we solve the optimization problem stated in \cref{prop:general_optimization}. The optimization can be reformulated as given in \cref{lemma:leakage_delta}.

\begin{lemma} \label{lemma:leakage_delta}
Considering PMFs of the form given in \cref{eq:dependent_on_0,eq:dependent_on_nz}, the total leakage $\totalleakagesdiff \triangleq \mathrm{L}_1+\mathrm{L}_2$ is given by
\begin{align*}
&\totalleakagesdiff = s \bigg[ \pz \bigg( \log \frac{\pz}{\sar} + \log \frac{\pz}{\sr} \bigg) 
+(q-1)\pzinv \bigg( \log \frac{\pzinv}{\sarinv} + \log \frac{\pzinv}{\srinv}\bigg) \bigg] \nonumber\\
& \!+\!(1-s) \!\cdot\! \bigg[ \pext \bigg( \log \frac{\pext}{\sarinv} + \log \frac{\pext}{\sr} \bigg) + \pnz \bigg( \log \frac{\pnz}{\sar} + \log \frac{\pnz}{\srinv} \bigg) +(q-2) \ptwoinv \bigg( \log \frac{\ptwoinv}{\sarinv} + \log \frac{\ptwoinv}{\srinv} \bigg)
\bigg],
\end{align*}
subject to
\begin{align}
    c_1(\pz,\pzinv) &\triangleq \pz + (q-1) \pzinv - 1 &&= 0, \label{eq:constraint1} \\
    c_2(\pext,\pnz,\pnzinv) &\triangleq \pext + \pnz + (q-2) \pnzinv - 1 &&= 0, \label{eq:constraint2} \\
    c_3(\pz,\pext) &\triangleq \pz s + \pext (1-s) - \savg + \sdiff &&= 0, \label{eq:constraint3} \\
    c_4(\pz,\pnz) &\triangleq \pz s + \pnz (1-s) - \savg - \sdiff &&= 0. \label{eq:constraint4}
\end{align}
where $\sr \triangleq \savg - \sdiff$, $\sar = \savg + \sdiff$, $\srinv \triangleq (1-\savg+\sdiff)/(q-1)$, $\sarinv \triangleq (1-\savg-\sdiff)/(q-1)$.
\begin{proof}
We obtain this result by expressing $\leakage{1}+\leakage{2}$ in terms of KL-divergences, using the distributions of given in \cref{eq:dependent_on_0,eq:dependent_on_nz}, and simplifying. %
\end{proof}
\end{lemma}

For clarity of presentation, we define the following quantities that will be helpful in stating the result of \cref{thm:optimal_pmf}.
\begin{align*}
\qfac & \triangleq (q-2)^2/(q-1), \alpha \triangleq s^2 (4+\qfac), \delta \triangleq -\qfac \savg^2,\\
\beta & \triangleq 4s(1-s-2\savg)-\qfac s (2\savg+s),\\
\gamma & \triangleq (1-s-2\savg)^2+\qfac(2s\savg + \savg^2).
\end{align*}

\begin{theorem} \label{thm:optimal_pmf_delta}
Given desired a desired average sparsity $\savg$, the optimal $\sdiff=0$ and the optimal PMF of the form given in \cref{eq:dependent_on_0,eq:dependent_on_nz} that minimizes the leakage is obtained by setting $\pz=\pz^\star$ which is the root of the polynomial $\alpha \pz^3 + \beta \pz^2 + \gamma \pz + \delta$ that satisfies $\max\{2\savg-1+s,0\} \leq 2 \pz s \leq 2\min\{s,\savg\}$. Having $\pz$, the remaining unknowns $\pzinv,\pext,\pnz$ and $\ptwoinv$ directly follow from \eqref{eq:constraint1}-\eqref{eq:constraint4}.
\begin{proof}
To determine the distribution of $\rvR$ given $\rvA$ that minimizes the leakage, we utilize the method of Lagrange multipliers to combine the objective function, i.e., the total leakage from \cref{lemma:leakage}, with the constraints in \eqref{eq:constraint1}-\eqref{eq:constraint4}. Thus, the objective function to be minimized can be expressed as
\begin{align*}
    \lossabbrev &\triangleq \losssdiff \\
    & = \totalleakagesdiff + \lambda_1 c_1(\pz,\pzinv) + \\
    & + \lambda_2 c_2(\pext,\pnz,\pnzinv) + \lambda_3 c_3(\pz,\pext) + \lambda_4 c_4(\pz,\pnz).
\end{align*}

This objective can be minimized by setting the gradient to zero, i.e., $\grad \lossabbrev = 0$, which amounts to solving a system of eleven equations with eleven unknowns. To continue the proof, we rely on the result of \cref{lemma:sdiff0,lemma:poly_result}.

\me{Show convexity of the optimization problem here..}

\begin{lemma} \label{lemma:sdiff0}
    Given desired a desired average sparsity $\savg=\frac{\sar+\sr}{2}$, where $\sar=\savg+\sdiff$ and $\sr=\savg-\sdiff$, with the objective in \cref{lemma:leakage_delta}, we obtain from $\nabla_{p_2,p_3,\sdiff} \lossabbrev = 0$ that the optimal $\sdiff$ is $0$.
\begin{proof}
We first state the system of equations given by $\nabla_{\pext,\pnz,\sdiff} \lossabbrev = 0$:
\begin{align}
    \frac{\partial \lossabbrev}{\partial \sdiff} &= s \left[ \pz \left(-\frac{1}{\sar} + \frac{1}{\sr}\right) + (q-1)\pzinv \left( \frac{1}{1-\sar} - \frac{1}{1-\sr}\right)\right] + \nonumber \\
    & + (1-s) \left[ p_2 \left( \frac{1}{1-\sar} + \frac{1}{\sr} \right) - p_3 \left( \frac{1}{\sar} + \frac{1}{1-\sr} \right) +  \right. \label{eqline:sys1} \\
    & \left. + (q-2) \ptwoinv \left( \frac{1}{1-\sar} - \frac{1}{1-\sr}\right) \right]  + \lambda_3 - \lambda_4 = 0 \label{eqline:partial_delta} \\
    \frac{\partial \lossabbrev}{\partial p_2} &= (1-s)\left(2\log(p_2) - \log(\sr) - \log(\sarinv) + 2\right) + \lambda_2 + (1-s) \lambda_3 = 0 \label{eqline:partial_p2} \\
    \frac{\partial \lossabbrev}{\partial p_3} &= (1-s)\left(2\log(p_3) - \log(\srinv) - \log(\sar) + 2\right) + \lambda_2 + (1-s) \lambda_4 = 0 \label{eqline:partial_p3}
\end{align}
We will first calculate $\lambda_3 - \lambda_4$ and subsequently the remaining parts. By computing $\eqref{eqline:partial_p2} - \eqref{eqline:partial_p3}$ and dividing the result by $(1-s)$, we obtain
\begin{align}
    &\lambda_3-\lambda_4 = 2 (\log(p_2) - \log(p_3)) + \log\left(\frac{\sarinv}{\sar}\right) + \log\left(\frac{\sr}{\srinv}\right) \label{eqline:lambda_diff1} \\
    &= 2\log\left(\frac{\savg-\sdiff-s p_1}{1-s}\right) - 2\log\left(\frac{\savg+\sdiff-s p_1}{1-s}\right) + \\
    &+ \log\left(\frac{1-\savg-\sdiff}{(q-1)(\savg+\sdiff)}\right) + \log\left(\frac{(q-1)(\savg-\sdiff)}{1-\savg+\sdiff}\right) \label{eqline:lambda_diff2} \\ 
    &= 2 \log\left(\frac{\savg-\sdiff-s p_1}{\savg+\sdiff-s p_1} \right) + \log\left(\frac{(1-\savg-\sdiff)(\savg-\sdiff)}{(1-\savg+\sdiff)(\savg+\sdiff)} \right) \leq 0, \label{eqline:lambda34}
\end{align}
where from \eqref{eqline:lambda_diff1} to \eqref{eqline:lambda_diff2} we used \eqref{eq:constraint3} and \eqref{eq:constraint4} to express $p_2$ and $p_3$ in terms of $p_1$, respectively.

Simplifying \eqref{eqline:sys1} by use of the constraints \cref{eq:constraint1,eq:constraint2,eq:constraint3,eq:constraint4} yields
\begin{align}
    &\frac{\partial \lossabbrev}{\partial \sdiff} - (\lambda_3 - \lambda_4) \nonumber \\
    &= \frac{1}{\sr} (s p_1 + (1-s) p_2) - \frac{1}{\sar} (s p_1 + (1-s)p_3)  + \nonumber \\
    & + \frac{1}{1-\sar} \underbrace{(s(q-1) \pzinv + (1-s) p_2 + (1-s)(q-2)\ptwoinv)}_{(a)} \nonumber \\
    & - \frac{1}{1-\sr} \underbrace{((q-1)\pzinv + (1-s)p_3 + (q-2)(1-s)\ptwoinv)}_{(b)} \\
    &= \frac{\sr}{\sr} -\frac{\sar}{\sar} + \frac{1-\sar}{1-\sar} - \frac{1-\sr}{1-\sr} = 0, \label{eqline:partial_sdiff_simplified}
\end{align}
where we used that $\sr = s p_1 + (1-s) p_2$ from \eqref{eq:constraint3}, $\sar = s p_1 + (1-s) p_3$ from \eqref{eq:constraint3}. Further, we obtain $1-\sar = (a)$ by solving \eqref{eq:constraint1} for $p_1$, substituting $p_1$ in \eqref{eq:constraint4} and solving for $p_3$ and finally inserting in \eqref{eq:constraint2}, multiplying by $(1-s)$ and solving for $1-\sar$. Lastly, we obtain $1-\sr = (b)$ by solving \eqref{eq:constraint1} for $p_1$, substituting $p_1$ in \eqref{eq:constraint3} and solving for $p_2$ and finally inserting in \eqref{eq:constraint2}, multiplying by $(1-s)$ and solving for $1-\sr$.
Putting \eqref{eqline:lambda34} and \eqref{eqline:partial_sdiff_simplified} together, we obtain
\begin{align}
    &\frac{\partial \lossabbrev}{\partial \sdiff} + \lambda_3 - \lambda_4 \\
    &= 2 \log\left(\frac{\savg-\sdiff-s p_1}{\savg+\sdiff-s p_1} \right) + \log\left(\frac{(1-\savg-\sdiff)(\savg-\sdiff)}{(1-\savg+\sdiff)(\savg+\sdiff)} \right) \leq 0. 
\end{align}
Thus, it follows that $\sdiff=0$.
\end{proof}
\end{lemma}

\begin{lemma} \label{lemma:poly_result}
Let $\sar$ and $\sr$ be the desired sparsities fo the shares $\bfR$ and $\bfA+\bfR$, and consider the objective given in \cref{lemma:leakage_delta}, we obtain from $\nabla_{\pz,\pzinv,\pext,\pnz,p_4,\pnzinv,\sdiff} \lossabbrev = 0$ the relation
\begin{align}
    \pz (\pnzinv)^2 &= \pzinv \pext \pnz. \label{eq:grad_obj_compact}
\end{align}
\begin{proof}
We apply \cref{lemma:sdiff0} and obtain that $\sdiff=0$. The system of equations $\nabla_{\pz,\pzinv,\pext,\pnz,p_4,\pnzinv} \lossabbrev = 0$ reads as follows.
\begin{align*}
    \frac{\partial \lossabbrev}{\partial p_1} &= s\left(2\log(p_1) - \log(\sr) - \log(\sar) + 2\right) + \lambda_1 + s\lambda_3 + s \lambda_4 = 0 \label{eqline:partial_p1} \\
    \frac{\partial \lossabbrev}{\partial p_1^{\text{inv}}} &= s(q-1)\left(2\log(p_1^{\text{inv}}) - \log(\srinv) - \log(\sarinv) + 2\right) + (q-1) \lambda_1 = 0 \label{eqline:partial_p1inv} \\
    \frac{\partial \lossabbrev}{\partial p_2} &= (1-s)\left(2\log(p_2) - \log(\sr) - \log(\sarinv) + 2\right) + \lambda_2 + (1-s) \lambda_3 = 0 \label{eqline:partial_p2} \\
    \frac{\partial \lossabbrev}{\partial p_3} &= (1-s)\left(2\log(p_3) - \log(\srinv) - \log(\sar) + 2\right) + \lambda_2 + (1-s) \lambda_4 = 0 \label{eqline:partial_p3} \\
    \frac{\partial \lossabbrev}{\partial p_{2,3}^\text{inv}} &= (1-s)(q-2) \left(2\log(\ptwoinv) - \log(\srinv) - \log(\sarinv) + 2\right) + (q-2) \lambda_2 = 0 \label{eqline:partial_p23inv}
\end{align*}
By scaling, we simplify and reformulate the system of equations and obtain
\begin{align}
    \frac{\partial \lossabbrev}{\partial p_1} &= 2\log(p_1) - \log(\sr) - \log(\sar) + 2 + \lambda_1^\prime + \lambda_3 + \lambda_4 = 0 \label{eqline:spartial_p1} \\
    \frac{\partial \lossabbrev}{\partial p_1^{\text{inv}}} &= 2\log(p_1^{\text{inv}}) - \log(\srinv) - \log(\sarinv) + 2 + \lambda_1^\prime = 0 \label{eqline:spartial_p1inv} \\
    \frac{\partial \lossabbrev}{\partial p_2} &= 2\log(p_2) - \log(\sr) - \log(\sarinv) + 2 + \lambda_2^\prime + \lambda_3 = 0 \label{eqline:spartial_p2} \\
    \frac{\partial \lossabbrev}{\partial p_3} &= 2\log(p_3) - \log(\srinv) - \log(\sar) + 2 + \lambda_2^\prime + \lambda_4 = 0 \label{eqline:spartial_p3} \\
    \frac{\partial \lossabbrev}{\partial p_{2,3}^\text{inv}} &= 2\log(\ptwoinv) - \log(\srinv) - \log(\sarinv) + 2 + \lambda_2^\prime = 0 \label{eqline:spartial_p23inv},
\end{align}
where $\lambda_1^\prime = \lambda_1/s$ and $\lambda_2^\prime = \lambda_2/(1-s)$. Calculating $\eqref{eqline:spartial_p1} - \eqref{eqline:spartial_p1inv} - \eqref{eqline:spartial_p2} - \eqref{eqline:spartial_p3} + 2 \cdot \eqref{eqline:spartial_p23inv} = 2\log\left(\frac{\pz {\ptwoinv}^2}{\pzinv, p_2 p_3}\right) = 0$, leading to the result stated in \cref{lemma:poly_result}.
\end{proof}
\end{lemma}

We solve \eqref{eq:constraint1}-\eqref{eq:constraint4} for $\pzinv,\pext,\pnz,\pnzinv$ in terms of $\pz$ (i.e., each a polynomial of degree one), which yields
\begin{align*}
    \pzinv &= \frac{1-\pz}{q-1} \\
    p_2 &= \frac{\sr - s\pz}{1-s} \\
    p_3 &= \frac{\sar - s\pz}{1-s} \\
    \ptwoinv &= \frac{1-s-\sar-\sr-2s\pz}{(1-s)(q-2)}.
\end{align*}
By inserting the equations into the result of \cref{lemma:poly_result}, we obtain a degree three polynomial in $\pz$, i.e.,
\begin{align}
    \pz (1-s-\sar-\sr-2s\pz)^2 - \frac{(1-\pz)(\sr - s\pz)(\sar - s\pz)}{(q-1)(1-s)^3(q-2)} = 0.
\end{align}
Thus, we seek to find the root of this polynomial in $\pz$ that satisfies the constraints given in the statement of \cref{thm:optimal_pmf_delta}. Since the problem is convex, the parameters yielding the local minimum must be a global minimizer to the constrained optimization problem.
\end{proof}
\end{theorem}

\begin{remark}
We prove that the minimum possible total leakage is obtained for $\sar = \sr$, i.e., according to \cref{lemma:sdiff0} if $\pext=\pnz$, and consequently when the leakages $\leakage{1}$ and $\leakage{2}$ are equal.
This result implies that the maximum leakage, i.e., $\max\{\leakage{1}, \leakage{2}\}$,is minimized for $\sr=\sar$ as well.
\end{remark}

